HATS-54b-HATS-58Ab: five new transiting hot Jupiters including one with a possible temperate companion

We report the discovery by the HATSouth project of 5 new transiting hot Jupiters (HATS-54b through HATS-58Ab). HATS-54b, HATS-55b and HATS-58Ab are prototypical short period ($P = 2.5-4.2$ days, $R_p\sim1.1-1.2$ $R_J$) hot-Jupiters that span effective temperatures from 1350 K to 1750 K, putting them in the proposed region of maximum radius inflation efficiency. The HATS-58 system is composed of two stars, HATS-58A and HATS-58B, which are detected thanks to Gaia DR2 data and which we account for in the joint modelling of the available data --- with this, we are led to conclude that the hot jupiter orbits the brighter HATS-58A star. HATS-57b is a short-period (2.35-day) massive (3.15 $M_J$) 1.14 $R_J$, dense ($2.65\pm0.21$ g cm$^{-3}$) hot-Jupiter, orbiting a very active star ($2\%$ peak-to-peak flux variability). Finally, HATS-56b is a short period (4.32-day) highly inflated hot-Jupiter (1.7 $R_J$, 0.6 $M_J$), which is an excellent target for future atmospheric follow-up, especially considering the relatively bright nature ($V=11.6$) of its F dwarf host star. This latter exoplanet has another very interesting feature: the radial velocities show a significant quadratic trend. If we interpret this quadratic trend as arising from the pull of an additional planet in the system, we obtain a period of $P_c = 815^{+253}_{-143}$ days for the possible planet HATS-56c, and a minimum mass of $M_c\sin i_c = 5.11 \pm 0.94$ $M_J$. The candidate planet HATS-56c would have a zero-albedo equilibrium temperature of $T_\textrm{eq}=332\pm 50$ K, and thus would be orbiting close to the habitable zone of HATS-56. Further radial-velocity follow-up, especially over the next two years, is needed to confirm the nature of HATS-56c.

==> HATS548-012_rvtable.tex <==
$ 7964.90759 $ & $  -458.04 $ & $    10.30 $ & $   10.0 $ & $   14.0 $ & $   0.303 $ & FEROS \\
$ 7971.92111 $ & $  -486.64 $ & $    10.30 $ & $    5.0 $ & $   14.0 $ & $   0.287 $ & FEROS \\
$ 7972.89572 $ & $   453.36 $ & $    14.10 $ & $   32.0 $ & $   18.0 $ & $   0.701 $ & FEROS \\
$ 7974.85803 $ & $   122.76 $ & $    13.90 $ & $  -44.0 $ & $   18.0 $ & $   0.536 $ & FEROS \\
$ 7979.88799 $ & $   382.66 $ & $    12.10 $ & $   51.0 $ & $   16.0 $ & $   0.676 $ & FEROS \\
$ 7980.87108 $ & $  -259.54 $ & $     9.50 $ & $   14.0 $ & $   13.0 $ & $   0.094 $ & FEROS \\
$ 7981.91787 $ & $   123.36 $ & $    10.90 $ & $   44.0 $ & $   15.0 $ & $   0.540 $ & FEROS \\
$ 7982.90648 $ & $   164.26 $ & $    10.30 $ & $   18.0 $ & $   14.0 $ & $   0.960 $ & FEROS \\
$ 7983.87763 $ & $  -315.54 $ & $    10.10 $ & $   45.0 $ & $   14.0 $ & $   0.373 $ & FEROS \\
$ 7984.84588 $ & $   482.36 $ & $    15.60 $ & $  -48.0 $ & $   20.0 $ & $   0.785 $ & FEROS \\
$ 7985.84967 $ & $  -515.34 $ & $    23.20 $ & $  112.0 $ & $   28.0 $ & $   0.212 $ & FEROS \\
$ 8032.81260 $ & $  -419.54 $ & $     9.30 $ & $   41.0 $ & $   12.0 $ & $   0.191 $ & FEROS \\
$ 8036.87243 $ & $   243.76 $ & $     9.40 $ & $   27.0 $ & $   12.0 $ & $   0.918 $ & FEROS \\
$ 8037.82663 $ & $  -424.04 $ & $    12.80 $ & $   52.0 $ & $   16.0 $ & $   0.324 $ & FEROS \\
$ 8038.82127 $ & $   440.66 $ & $    10.90 $ & $   36.0 $ & $   14.0 $ & $   0.747 $ & FEROS \\


==> HATS602-072_rvtable.tex <==
$ 7069.70274 $ & $   -94.56 $ & $    16.00 $ & $    9.0 $ & $   24.0 $ & $   0.313 $ & HARPS \\
$ 7070.69336 $ & $    54.44 $ & $    16.00 $ & $  -54.0 $ & $   24.0 $ & $   0.549 $ & HARPS \\
$ 7071.67030 $ & $    96.44 $ & $    12.00 $ & $   26.0 $ & $   17.0 $ & $   0.781 $ & HARPS \\
$ 7072.65330 $ & $   -10.56 $ & $    21.00 $ & $   18.0 $ & $   27.0 $ & $   0.015 $ & HARPS \\
$ 7119.60123 $ & $  -113.56 $ & $    19.00 $ & $  -92.0 $ & $   27.0 $ & $   0.182 $ & HARPS \\
$ 7120.58327 $ & $   -37.56 $ & $    24.00 $ & $  -78.0 $ & $   31.0 $ & $   0.415 $ & HARPS \\
$ 7331.79680 $ & $    66.44 $ & $    20.00 $ & $   78.0 $ & $   27.0 $ & $   0.654 $ & HARPS \\
$ 7332.82189 $ & $    60.44 $ & $    14.00 $ & $  -20.0 $ & $   21.0 $ & $   0.898 $ & HARPS \\


==> HATS698-034_rvtable.tex <==
$ 7768.73601 $ & $    42.88 $ & $    17.40 $ & $  105.0 $ & $   14.0 $ & $   0.545 $ & FEROS \\
$ 7796.68850 $ & $    -4.07 $ & $    10.50 $ & $  113.0 $ & $   10.0 $ & $   0.008 $ & FEROS \\
$ 7801.88207 $ & $   -50.01 $ & $    15.20 $ & $  133.0 $ & $   13.0 $ & $   0.209 $ & FEROS \\
$ 7803.87790 $ & $    31.05 $ & $    11.30 $ & $  105.0 $ & $   10.0 $ & $   0.671 $ & FEROS \\
$ 7804.76141 $ & $    43.23 $ & $    10.60 $ & $  119.0 $ & $   10.0 $ & $   0.875 $ & HARPS \\
$ 7805.79949 $ & $   -43.34 $ & $     9.30 $ & $  151.0 $ & $    9.0 $ & $   0.115 $ & HARPS \\
$ 7806.82285 $ & $   -60.47 $ & $    19.00 $ & $  110.0 $ & $   18.0 $ & $   0.352 $ & HARPS \\
$ 7809.88240 $ & $   -42.12 $ & $    13.30 $ & $  118.0 $ & $   11.0 $ & $   0.059 $ & FEROS \\
$ 7810.78947 $ & $   -65.04 $ & $    11.00 $ & $   82.0 $ & $   10.0 $ & $   0.269 $ & FEROS \\
$ 7812.80965 $ & $    40.61 $ & $    11.60 $ & $   94.0 $ & $   10.0 $ & $   0.736 $ & FEROS \\
$ 7814.84266 $ & $   -50.74 $ & $    11.40 $ & $   78.0 $ & $   10.0 $ & $   0.206 $ & FEROS \\
$ 7829.60532 $ & $    33.78 $ & $    11.90 $ & $   90.0 $ & $   11.0 $ & $   0.620 $ & FEROS \\
$ 7829.72742 $ & $    57.80 $ & $    12.00 $ & $  149.0 $ & $   11.0 $ & $   0.648 $ & FEROS \\
$ 7834.69030 $ & $    61.15 $ & $    11.00 $ & $  103.0 $ & $   10.0 $ & $   0.795 $ & FEROS \\
$ 7835.77029 $ & $     7.73 $ & $    13.60 $ & $  151.0 $ & $   12.0 $ & $   0.045 $ & FEROS \\
$ 7836.69418 $ & $   -31.26 $ & $    13.70 $ & $  121.0 $ & $   12.0 $ & $   0.259 $ & FEROS \\
$ 7837.61306 $ & $   -29.83 $ & $    13.70 $ & $   90.0 $ & $   12.0 $ & $   0.471 $ & FEROS \\
$ 7843.77804 $ & $    15.56 $ & $    13.00 $ & $   86.0 $ & $   11.0 $ & $   0.897 $ & FEROS \\
$ 7844.62448 $ & $   -32.17 $ & $    12.30 $ & $   97.0 $ & $   11.0 $ & $   0.092 $ & FEROS \\
$ 7902.69762 $ & $    26.35 $ & $    16.90 $ & $   95.0 $ & $   14.0 $ & $   0.521 $ & FEROS \\
$ 7905.61364 $ & $   -76.07 $ & $    11.60 $ & $  111.0 $ & $   11.0 $ & $   0.195 $ & FEROS \\
$ 7907.66550 $ & $    54.25 $ & $    15.50 $ & $   96.0 $ & $   13.0 $ & $   0.669 $ & FEROS \\
$ 7909.56595 $ & $   -43.57 $ & $    13.00 $ & $   55.0 $ & $   11.0 $ & $   0.109 $ & FEROS \\
$ 7910.56691 $ & $   -66.16 $ & $    13.20 $ & $  112.0 $ & $   11.0 $ & $   0.340 $ & FEROS \\
$ 7911.67981 $ & $    30.26 $ & $    16.30 $ & $  142.0 $ & $   13.0 $ & $   0.597 $ & FEROS \\
$ 7913.66972 $ & $   -13.28 $ & $    23.20 $ & $   50.0 $ & $   17.0 $ & $   0.058 $ & FEROS \\
$ 7914.57791 $ & $   -71.47 $ & $    14.40 $ & $   54.0 $ & $   12.0 $ & $   0.268 $ & FEROS \\
$ 7915.52162 $ & $   -25.48 $ & $    10.60 $ & $   96.0 $ & $   10.0 $ & $   0.486 $ & FEROS \\
$ 7943.53037 $ & $   -37.36 $ & $    11.80 $ & $   86.0 $ & $   11.0 $ & $   0.962 $ & FEROS \\
$ 7944.57253 $ & $  -103.15 $ & $    12.40 $ & $  138.0 $ & $   11.0 $ & $   0.203 $ & FEROS \\
$ 7945.56468 $ & $   -58.69 $ & $    13.50 $ & $  149.0 $ & $   12.0 $ & $   0.433 $ & FEROS \\
$ 7946.58367 $ & $    26.85 $ & $    13.10 $ & $  145.0 $ & $   11.0 $ & $   0.668 $ & FEROS \\
$ 7948.60621 $ & $    27.86 $ & $    20.80 $ & $  115.0 $ & $   16.0 $ & $   0.136 $ & FEROS \\
$ 7949.61253 $ & $   -46.77 $ & $    23.40 $ & $   50.0 $ & $   18.0 $ & $   0.368 $ & FEROS \\
$ 7964.49356 $ & $    57.71 $ & $    19.50 $ & $  185.0 $ & $   15.0 $ & $   0.809 $ & FEROS \\
$ 7966.51932 $ & $   -93.54 $ & $    14.00 $ & $   80.0 $ & $   12.0 $ & $   0.278 $ & FEROS \\
$ 7972.49885 $ & $    46.05 $ & $    13.70 $ & $   93.0 $ & $   12.0 $ & $   0.660 $ & FEROS \\
$ 7973.49841 $ & $    48.98 $ & $    20.50 $ & $  113.0 $ & $   16.0 $ & $   0.892 $ & FEROS \\
$ 7975.50082 $ & $   -34.63 $ & $    33.70 $ & $  197.0 $ & $   25.0 $ & $   0.355 $ & FEROS \\
$ 7980.48538 $ & $   -50.37 $ & $    14.20 $ & $  102.0 $ & $   12.0 $ & $   0.507 $ & FEROS \\
$ 7981.49226 $ & $   -31.98 $ & $    13.90 $ & $   53.0 $ & $   12.0 $ & $   0.740 $ & FEROS \\
$ 7982.48565 $ & $   -38.78 $ & $    12.50 $ & $   99.0 $ & $   11.0 $ & $   0.970 $ & FEROS \\
$ 7983.48566 $ & $  -100.48 $ & $    12.30 $ & $  113.0 $ & $   11.0 $ & $   0.201 $ & FEROS \\
$ 8096.76533 $ & $   -77.55 $ & $    11.50 $ & $   88.0 $ & $   10.0 $ & $   0.394 $ & FEROS \\
$ 8109.85445 $ & $   -21.52 $ & $    13.20 $ & $   90.0 $ & $   11.0 $ & $   0.421 $ & FEROS \\
$ 8112.83173 $ & $   -46.41 $ & $    11.40 $ & $  102.0 $ & $   10.0 $ & $   0.109 $ & FEROS \\
$ 8113.86302 $ & $   -75.60 $ & $    11.20 $ & $  104.0 $ & $   10.0 $ & $   0.348 $ & FEROS \\
$ 8135.86022 $ & $   -31.29 $ & $    12.00 $ & $   79.0 $ & $   11.0 $ & $   0.434 $ & FEROS \\
$ 8137.86692 $ & $   -10.99 $ & $    12.00 $ & $   59.0 $ & $   11.0 $ & $   0.898 $ & FEROS \\
$ 8141.87523 $ & $    49.60 $ & $    15.40 $ & $  100.0 $ & $   13.0 $ & $   0.825 $ & FEROS \\
$ 8143.80200 $ & $   -94.07 $ & $    13.10 $ & $  140.0 $ & $   11.0 $ & $   0.270 $ & FEROS \\
$ 8144.68258 $ & $   -34.95 $ & $    11.70 $ & $  114.0 $ & $   11.0 $ & $   0.474 $ & FEROS \\
$ 8145.88228 $ & $    17.60 $ & $    12.80 $ & $   91.0 $ & $   11.0 $ & $   0.751 $ & FEROS \\
$ 8148.88292 $ & $   -47.14 $ & $    11.40 $ & $  120.0 $ & $   10.0 $ & $   0.445 $ & FEROS \\
$ 8151.76621 $ & $   -61.30 $ & $    12.10 $ & $   82.0 $ & $   11.0 $ & $   0.112 $ & FEROS \\
$ 8160.72106 $ & $   -39.10 $ & $    13.80 $ & $  101.0 $ & $   12.0 $ & $   0.182 $ & FEROS \\
$ 8166.89247 $ & $    35.14 $ & $    11.70 $ & $  101.0 $ & $   11.0 $ & $   0.609 $ & FEROS \\
$ 8170.82889 $ & $   -11.54 $ & $    11.00 $ & $   70.0 $ & $   10.0 $ & $   0.520 $ & FEROS \\
$ 8200.69631 $ & $    20.61 $ & $    11.70 $ & $  138.0 $ & $   11.0 $ & $   0.426 $ & FEROS \\


==> HATS700-017_rvtable.tex <==
$ 7120.76007 $ & $    68.29 $ & $    19.00 $ & $   15.0 $ & $   31.0 $ & $   0.879 $ & HARPS \\
$ 7181.50030 $ & $   115.34 $ & $    13.00 $ & $   24.0 $ & $   18.0 $ & $   0.753 $ & FEROS \\
$ 7182.69946 $ & $  -196.66 $ & $    15.00 $ & $  -56.0 $ & $   20.0 $ & $   0.225 $ & FEROS \\
$ 7185.49965 $ & $  -133.66 $ & $    14.00 $ & $  -59.0 $ & $   19.0 $ & $   0.325 $ & FEROS \\
$ 7186.66323 $ & $   -50.66 $ & $    23.00 $ & $   14.0 $ & $   30.0 $ & $   0.782 $ & FEROS \\
$ 7187.66100 $ & $  -141.66 $ & $    15.00 $ & $  -50.0 $ & $   20.0 $ & $   0.175 $ & FEROS \\
$ 7195.53227 $ & $   -64.66 $ & $    15.00 $ & $   15.0 $ & $   20.0 $ & $   0.268 $ & FEROS \\
$ 7224.61924 $ & $   126.34 $ & $    23.00 $ & $  157.0 $ & $   30.0 $ & $   0.701 $ & FEROS \\
$ 7228.51247 $ & $   -47.66 $ & $    16.00 $ & $   84.0 $ & $   21.0 $ & $   0.231 $ & FEROS \\
$ 7232.53561 $ & $     6.34 $ & $    21.00 $ & $   40.0 $ & $   25.0 $ & $   0.813 $ & FEROS \\
$ 7887.75568 $ & $    20.19 $ & $    43.10 $ & $  -51.0 $ & $   57.0 $ & $   0.349 $ & HARPS \\
$ 7888.76435 $ & $   161.59 $ & $    59.00 $ & $    6.0 $ & $   77.0 $ & $   0.746 $ & HARPS \\
$ 7903.67827 $ & $   -75.86 $ & $    26.50 $ & $  -84.0 $ & $   34.0 $ & $   0.608 $ & FEROS \\
$ 7905.74906 $ & $  -146.16 $ & $    14.70 $ & $    4.0 $ & $   20.0 $ & $   0.421 $ & FEROS \\
$ 7906.67308 $ & $   180.54 $ & $    12.60 $ & $    3.0 $ & $   18.0 $ & $   0.785 $ & FEROS \\
$ 7907.58913 $ & $   -76.76 $ & $    12.30 $ & $ -129.0 $ & $   17.0 $ & $   0.145 $ & FEROS \\
$ 7908.61270 $ & $    91.74 $ & $    15.10 $ & $   36.0 $ & $   20.0 $ & $   0.547 $ & FEROS \\
$ 7911.51620 $ & $    92.54 $ & $    14.30 $ & $  -33.0 $ & $   19.0 $ & $   0.688 $ & FEROS \\
$ 7913.54999 $ & $     8.84 $ & $    15.30 $ & $  -48.0 $ & $   19.0 $ & $   0.488 $ & FEROS \\
$ 7914.54968 $ & $   103.74 $ & $    13.10 $ & $  -64.0 $ & $   18.0 $ & $   0.881 $ & FEROS \\
$ 7915.61554 $ & $  -104.86 $ & $    12.60 $ & $   -4.0 $ & $   17.0 $ & $   0.299 $ & FEROS \\
$ 7943.48406 $ & $   -63.86 $ & $    11.50 $ & $  -22.0 $ & $   16.0 $ & $   0.253 $ & FEROS \\
$ 7944.53353 $ & $   147.34 $ & $    11.80 $ & $   10.0 $ & $   16.0 $ & $   0.666 $ & FEROS \\
$ 7945.60475 $ & $     7.24 $ & $    14.40 $ & $  -62.0 $ & $   19.0 $ & $   0.087 $ & FEROS \\
$ 7946.50173 $ & $   -43.96 $ & $    12.70 $ & $   50.0 $ & $   18.0 $ & $   0.439 $ & FEROS \\
$ 7948.62577 $ & $   -92.56 $ & $    23.00 $ & $  -24.0 $ & $   28.0 $ & $   0.274 $ & FEROS \\
$ 7949.63156 $ & $   156.44 $ & $    24.60 $ & $  193.0 $ & $   32.0 $ & $   0.670 $ & FEROS \\
$ 7964.52884 $ & $     2.04 $ & $    18.40 $ & $   83.0 $ & $   25.0 $ & $   0.525 $ & FEROS \\
$ 7966.57374 $ & $   -58.46 $ & $    20.10 $ & $  108.0 $ & $   26.0 $ & $   0.329 $ & FEROS \\
$ 7967.50871 $ & $   176.74 $ & $    33.10 $ & $   95.0 $ & $   34.0 $ & $   0.696 $ & FEROS \\
$ 7969.51414 $ & $    35.44 $ & $    18.70 $ & $  -31.0 $ & $   25.0 $ & $   0.485 $ & FEROS \\
$ 7970.52194 $ & $   152.64 $ & $    16.30 $ & $  -82.0 $ & $   22.0 $ & $   0.881 $ & FEROS \\
$ 7971.52200 $ & $   -77.06 $ & $    14.40 $ & $   66.0 $ & $   19.0 $ & $   0.274 $ & FEROS \\
$ 7972.53369 $ & $   135.74 $ & $    15.70 $ & $   26.0 $ & $   20.0 $ & $   0.671 $ & FEROS \\


==> HATS737-002_rvtable.tex <==
$ 7734.84067 $ & $    61.42 $ & $    19.30 $ & $   27.0 $ & $   15.0 $ & $   0.375 $ & FEROS \\
$ 7803.86422 $ & $    68.82 $ & $    11.40 $ & $   21.0 $ & $   10.0 $ & $   0.739 $ & FEROS \\
$ 7804.80057 $ & $    36.10 $ & $    10.40 $ & $   50.0 $ & $    9.0 $ & $   0.961 $ & HARPS \\
$ 7805.82841 $ & $   -64.00 $ & $    13.10 $ & $   26.0 $ & $   12.0 $ & $   0.204 $ & HARPS \\
$ 7806.84926 $ & $   -21.90 $ & $    16.80 $ & $    4.0 $ & $   15.0 $ & $   0.446 $ & HARPS \\
$ 7809.86928 $ & $    -8.18 $ & $    13.20 $ & $   24.0 $ & $   11.0 $ & $   0.162 $ & FEROS \\
$ 7810.58776 $ & $  -103.38 $ & $    14.80 $ & $    1.0 $ & $   12.0 $ & $   0.332 $ & FEROS \\
$ 7812.82176 $ & $    72.92 $ & $    12.30 $ & $    8.0 $ & $   11.0 $ & $   0.862 $ & FEROS \\
$ 7814.80930 $ & $    32.52 $ & $    12.10 $ & $   38.0 $ & $   10.0 $ & $   0.333 $ & FEROS \\
$ 7815.84641 $ & $   -13.68 $ & $    11.50 $ & $   -8.0 $ & $   10.0 $ & $   0.579 $ & FEROS \\
$ 7829.71397 $ & $   -37.58 $ & $    12.30 $ & $  -57.0 $ & $   11.0 $ & $   0.867 $ & FEROS \\
$ 7831.74171 $ & $   -63.48 $ & $    14.30 $ & $   -8.0 $ & $   12.0 $ & $   0.348 $ & FEROS \\
$ 7832.70462 $ & $    45.12 $ & $    14.40 $ & $   19.0 $ & $   12.0 $ & $   0.576 $ & FEROS \\
$ 7835.72891 $ & $   -17.98 $ & $    14.60 $ & $   60.0 $ & $   12.0 $ & $   0.293 $ & FEROS \\
$ 7866.56935 $ & $    40.40 $ & $     6.60 $ & $   53.0 $ & $    6.0 $ & $   0.604 $ & HARPS \\
$ 7867.58943 $ & $    37.60 $ & $     8.50 $ & $   17.0 $ & $    8.0 $ & $   0.846 $ & HARPS \\
$ 7869.47820 $ & $   -74.60 $ & $    11.10 $ & $   38.0 $ & $   10.0 $ & $   0.294 $ & HARPS \\
$ 7869.48251 $ & $   -74.60 $ & $    11.10 $ & $   38.0 $ & $   10.0 $ & $   0.295 $ & HARPS \\
$ 7870.56130 $ & $    34.40 $ & $     6.60 $ & $   29.0 $ & $    6.0 $ & $   0.551 $ & HARPS \\
$ 7871.58342 $ & $    51.90 $ & $     9.70 $ & $   34.0 $ & $    9.0 $ & $   0.793 $ & HARPS \\


==> makefile <==
TARGET=hats54-58
PRINTER=peyton_color
SUB=submit_v1
CURRENTDIR=$(shell pwd | sed -e 's|.*/||g')
VERSION=$(shell ls -l $(TARGET).tex | \
	sed -e 's|.*->||g' -e 's|.*_V||g' -e 's|.tex||g')


all: $(TARGET).pdf

.PHONY: all clean save print show


show:
	@echo VERSION: $(VERSION)

$(TARGET).dvi: *.tex *.cls *.bib
	sed -e "s|HATVERSION|$(VERSION)|g" emulateapj_template.cls > emulateapj.cls
	latex $(TARGET).tex
	latex $(TARGET).tex
	bibtex $(TARGET)
	latex $(TARGET).tex
	latex $(TARGET).tex
	latex $(TARGET).tex

$(TARGET).ps: $(TARGET).dvi
	dvips -t letter $(TARGET).dvi -o

$(TARGET).pdf: $(TARGET).ps
	ps2pdf $< $@

save:
	tar cvzf ../$(TARGET)_V$(VERSION).tgz ../$(CURRENTDIR)/
	#gzip $(TARGET).tar
	#mv $(TARGET).tar.gz $(TARGET).tgz

sub:
	test -d $(SUB) || mkdir $(SUB)
	test -d $(SUB)/img || mkdir $(SUB)/img
	cp $(TARGET).tex $(SUB)/hatpxx.tex
	cp img/*.eps $(SUB)/img

clean:
	rm -f $(TARGET).ps \
	$(TARGET).dvi \
	$(TARGET).aux \
	$(TARGET).log \
	$(TARGET).pdf \
	$(TARGET).idx \
	$(TARGET).inx \
	$(TARGET).toc \
	$(TARGET).tgz
	
print: $(TARGET).ps
	lpr -P$(PRINTER) $<
	


==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxB below with a unique identifier for each planet (e.g. xxxxB for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxB. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxB}{HATS-40}
\newcommand{\hatcurbxxxxB}{HATS-40b}
\newcommand{\hatcurcxxxxB}{HATS-40c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxB}{40}

\newcommand{\hatcurCCtwomassshortxxxxB}{06421710-2946365}

%\newcommand{\hatcurCCraxxxxB}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxB}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxB}{\hatcurRVgamma{\hatcurplanetnumxxxxB}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxB}{\hatcurRVgamma{\hatcurplanetnumxxxxB}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxB}{\ensuremath{NULL\pm NULL}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxB}{i}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxB}{YY}
%\newcommand{\hatcurisoshortxxxxB}{Baraffe}
\newcommand{\hatcurisofullxxxxB}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxB}{Baraffe}
\newcommand{\hatcurisocitexxxxB}{yi:2001}
%\newcommand{\hatcurisocitexxxxB}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxB}{\arstar}
%\newcommand{\hatcurlumindxxxxB}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxB}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxB}{BB}
%\newcommand{\hatcurjhkfilsetxxxxB}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxBx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxB}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEzfehxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxB}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEzfehshortxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxB}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEloggxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxB}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvsinxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxB}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvmacxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxB}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvmicxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxB}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxB}}}

